Bouncing Scenario and Cosmic Dynamics in Modified Theories of Gravity

The main objective of this study is to investigate the phenomenon of the bouncing scenario of the universe. The most widely recognized cosmological framework is the standard cosmological model, sometimes referred to as the Big Bang model. This is mainly because of its inherent properties and its consistent alignment with recent observational studies. However, the standard cosmological model faces some challenges concerning the physical conditions at the initial epochs. Some of these issues include the initial singularity problem, flatness problem, horizon problem, etc. Some of these challenges could potentially be addressed by incorporating the inflationary scenario into the cosmological framework of the universe. However, the inflationary mechanism is not able to tackle the occurrence of the initial singularity. The bouncing cosmology offers a probable solution to this initial singularity issue. In addition, it is capable of addressing some other issues that may arise during the early stages. Hence, in the modified gravity theory, bounce cosmology has been discussed.

==> Appendice/Appendices.tex <==
% Appendix Template

\chapter{Appendices} % Main appendix title

\label{AppendixX} % Change X to a consecutive letter; for referencing this appendix elsewhere, use \ref{AppendixX}

\lhead{Appendix X. \emph{Appendix Title Here}} % Change X to a consecutive letter; this is for the header on each page - perhaps a shortened title
\textbf{Bianchi Type-III calculations}\\
For the line element (\ref{ch2met1}) the components of metric tensor $g_{\mu \nu}$ are\\

$g_{\mu \nu }=\left(
\begin{array}{cccc}
 1 & 0 & 0 & 0 \\
 0 & -A(t)^2 & 0 & 0 \\
 0 & 0 & -B(t)^2 & 0 \\
 0 & 0 & 0 & -B(t)^2 \\
\end{array}
\right)$
and 
$g^{\mu \nu }=\left(
\begin{array}{cccc}
 1 & 0 & 0 & 0 \\
 0 & -\frac{1}{A(t)^2} & 0 & 0 \\
 0 & 0 & -\frac{1}{B(t)^2} & 0 \\
 0 & 0 & 0 & -\frac{1}{B(t)^2} \\
\end{array}
\right)$\\

The non-vanishing Christoffel's symbols of the second kind for the line element (\ref{ch2met1}) are
\begin{eqnarray*}
 \text{$\Gamma$ [0, 1, 1]} = A(t) \dot{A}(t),   
 \text{$\Gamma$ [0, 2, 2]} = B(t) \dot{B}(t),  
 \text{$\Gamma$ [0, 3, 3]} = B(t) \dot{B}(t), \\
 \text{$\Gamma$ [1, 1, 0]} = \frac{\dot{A}(t)}{A(t)},  
 \text{$\Gamma$ [2, 2, 0]} = \frac{\dot{B}(t)}{B(t)},   
 \text{$\Gamma$ [3, 3, 0]} = \frac{\dot{B}(t)}{B(t)} 
\end{eqnarray*}
The non-vanishing components of $R_{\mu \nu}$ for the line element (\ref{ch2met1}) are

$\text{R[0, 0]} = -\frac{\ddot{A}(t)}{A(t)}-\frac{2 \ddot{B}(t)}{B(t)}$, $\text{R[1, 1]} = A(t) \left(\frac{2 \dot{A}(t) \dot{B}(t)}{B(t)}+\dot{A}(t)\right)$,\\
 $\text{R[2, 2]} = \dot{B}(t)^2+\frac{B(t) \dot{A}(t) \dot{B}(t)}{A(t)}+B(t) \dot{B}(t)$, $\text{R[3, 3]}= \dot{B}(t)^2+\frac{B(t) \dot{A}(t) \dot{B}(t)}{A(t)}+B(t) \dot{B}(t)$
%\begin{eqnarray*}
% \text{R[1, 1]} &=& -\frac{A''(t)}{A(t)}-\frac{2 B''(t)}{B(t)} \\
% \text{R[2, 2]} & A(t) \left(\frac{2 A'(t) B'(t)}{B(t)}+A''(t)\right) \\
% \text{R[3, 3]} & B'(t)^2+\frac{B(t) A'(t) B'(t)}{A(t)}+B(t) B''(t) \\
% \text{R[4, 4]} & B'(t)^2+\frac{B(t) A'(t) B'(t)}{A(t)}+B(t) B''(t) \\
%\end{eqnarray*}





==> Makefile <==
# Makefile for BPHC Latex Report Class

LATEXMK=latexmk
LATEXOPT=-jobname="Thesis" -file-line-error
MAIN=main
THESIS=$(MAIN).tex
SOURCES=$(THESIS) Makefile

.PHONY: clean FORCE all

all: 	$(MAIN).pdf

cont: FORCE
	$(LATEXMK) -f -pdf -pvc $(LATEXOPT) $(THESIS)

$(thesis): FORCE
	latexmk -pdf -f $(thesis)

$(MAIN).pdf: .refresh $(SOURCES)
	$(LATEXMK) -f -pdf $(LATEXOPT) $(THESIS)

clean:
	$(LATEXMK) -c $(MAIN).tex
	find . \( -name "*.toc" -o -name "*.fdb_latexmk" \
							-o -name "*.pdfsync" \
                            -o -name "*.log" \
                            -o -name "*.fls" \
                            -o -name "*.aux" \
                            -o -name "*.bbl" \
                            -o -name "*.blg" \
                            -o -name "*.glo" \
                            -o -name "*.ist" \
                            -o -name "*.lof" \
                            -o -name "*.lot" \
                            -o -name "*.out" \
                            -o -name "*.toc" \
                            \) -print0 | xargs -0 rm -f

FORCE:
	touch .refresh
	$(MAKE) $(MAIN).pdf

.refresh:
	touch .refresh

